Sparse Attentive Backtracking: Temporal CreditAssignment Through Reminding

Learning long-term dependencies in extended temporal sequences requires credit assignment to events far back in the past. The most common method for training recurrent neural networks, back-propagation through time (BPTT), requires credit information to be propagated backwards through every single step of the forward computation, potentially over thousands or millions of time steps. This becomes computationally expensive or even infeasible when used with long sequences. Importantly, biological brains are unlikely to perform such detailed reverse replay over very long sequences of internal states (consider days, months, or years.) However, humans are often reminded of past memories or mental states which are associated with the current mental state. We consider the hypothesis that such memory associations between past and present could be used for credit assignment through arbitrarily long sequences, propagating the credit assigned to the current state to the associated past state. Based on this principle, we study a novel algorithm which only back-propagates through a few of these temporal skip connections, realized by a learned attention mechanism that associates current states with relevant past states. We demonstrate in experiments that our method matches or outperforms regular BPTT and truncated BPTT in tasks involving particularly long-term dependencies, but without requiring the biologically implausible backward replay through the whole history of states. Additionally, we demonstrate that the proposed method transfers to longer sequences significantly better than LSTMs trained with BPTT and LSTMs trained with full self-attention.

==> tmp.tex <==


    
% --- original copying T=100 table
%\begin{table*}[h!]
%\label{copy100}
%\footnotesize
%\centering
%\vspace{-0.5\baselineskip}
%\begin{tabular}{l||cccc}
%\toprule
%\textbf {Method} &  \textbf{Length (T)} & \textbf{Accuracy ($\%$)} &    \textbf{CE (last 10 chars)} & \textbf{CE}   \\ 
%\midrule
%LSTM (full BPTT) & 100 & 98.8 & 0.030 & 0.002  \\
%LSTM (full self-attention) & 100 & 100.0 & 0.0008 & 0.0000 \\
%\midrule
%LSTM (TBPTT, $k_\textrm{trunc}$= 5) & 100 & 31.0 & 1.737 & 0.145\\ 
%LSTM (TBPTT, $k_\textrm{trunc}$ = 10) & 100 &  29.6 & 1.772 & 0.148 \\ 
%LSTM (TBPTT, $k_\textrm{trunc}$ = 20) & 100 & 30.5 & 1.714 & 0.143\\ 
%\midrule
%\gls{SAB} ($k_\textrm{trunc}$=1, $k_\textrm{top}$=1)   & 100 & 57.9 &   1.041 & 0.087 \\
%%\gls{SAB} ($k_\textrm{trunc}$=1, $k_\textrm{top}$=1)   & 100 & 17.6 &   2.044 & 0.170 \\
%\gls{SAB} ($k_\textrm{trunc}$=1, $k_\textrm{top}$=5)   & 100 & {\bf 100.0} & {\bf 0.001} & {\bf 0.000}    \\
%%\gls{SAB} ($k_\textrm{trunc}$=1, $k_\textrm{top}$=10)   & 100 & 62.7 & 0.964 & 0.080    \\
%\gls{SAB} ($k_\textrm{trunc}$=5, $k_\textrm{top}$=5)   & 100 & {\bf 100.0} & {\bf 0.000} & {\bf 0.000}  \\
%%\gls{SAB} ($k_\textrm{trunc}$=5, $k_\textrm{top}$=5)   & 100 & 99.6 & 0.017 & 0.001  \\
%\gls{SAB} ($k_\textrm{trunc}$=10, $k_\textrm{top}$=10) & 100 & {\bf100.0} & {\bf 0.000} & {\bf 0.001}    \\
%\midrule
%\textbf{Ablation study}  &  &  &  & \\
%\midrule
%\gls{SAB} (no MU) ($k_\textrm{trunc}$=1, $k_\textrm{top}$=1) & 100 & 49.0 & 1.252 & 0.104    \\
%\gls{SAB} (no MU) ($k_\textrm{trunc}$=5, $k_\textrm{top}$=5) & 100 & 98.3 & 0.042 & 0.0036   \\
%\gls{SAB} (no MU) ($k_\textrm{trunc}$=10, $k_\textrm{top}$=10) & 100 & 99.6 & 0.022 & 0.0018   \\
%\midrule
%\gls{SAB} ($k_\textrm{trunc}$=5, $k_\textrm{top}$=all) & 100 & 40.5 & 1.529  &  0.127  \\
%\gls{SAB} ($k_\textrm{trunc}$=10, $k_\textrm{top}$=all) & 100 &  &   &    \\
%\bottomrule
%\end{tabular}
%%\vspace{-1\baselineskip}
%\vspace{-1mm}
%\caption{Test accuracy and cross-entropy (CE) loss performance on the {\bf copying task} with sequence lengths of $T = 100$} %Models that use TBPTT cannot solve this task while \gls{SAB} and BPTT can both achieve optimal performance.}
%\label{tab:copy100}
%\end{table*}

% ----- original copying T=200 table
%\begin{table*}[h!]
%\footnotesize
%\label{copy200}
%\begin{center}
%\begin{tabular}{l||cccc}
%\toprule
%\textbf{Method} &  \textbf{Length (T)} & \textbf{Accuracy ($\%$)} &     \textbf{CE (last 10 chars)} & \textbf{CE}  \\ 
%\midrule
%LSTM (full BPTT)  & 200 & 56.0 & 1.07 & 0.046 \\ 
%LSTM (full selfattention) & 200 & 100.0 & 0.001 & 0.000  \\
%\midrule
%LSTM (TBPTT, $k_\textrm{trunc}$=  5) & 200  & 17.1  & 2.03 & 0.092 \\
%LSTM (TBPTT, $k_\textrm{trunc}$= 10) & 200  & 20.2 & 1.98 & 0.090 \\ 
%LSTM (TBPTT, $k_\textrm{trunc}$= 20) &  200 & 35.8 & 1.61 & 0.073 \\ 
%LSTM (TBPTT, $k_\textrm{trunc}$=150) & 200 & 35.0 & 1.596 & 0.073 \\
%\midrule
%\gls{SAB} ($k_\textrm{trunc}$=1, $k_\textrm{top}$=1)   & 200 & 39.9 & 1.516 & 0.069 \\
%%\gls{SAB} ($k_\textrm{trunc}$=1, $k_\textrm{top}$=1)   & 200 & 29.8 & 1.818 & 0.083 \\
%\gls{SAB} ($k_\textrm{trunc}$=5, $k_\textrm{top}$=5)   & 200 & {\bf 100.0} & {\bf 0.000} & {\bf 0.000} \\
%%\gls{SAB} ($k_\textrm{trunc}$=5, $k_\textrm{top}$=5)   & 200 & {\bf 99.3} & {\bf 0.032} & {\bf 0.001} \\
%\gls{SAB} ($k_\textrm{trunc}$=10, $k_\textrm{top}$=10) & 200 & {\bf 100.0} & {\bf 0.000} & {\bf 0.000} \\
%%\gls{SAB} ($k_\textrm{trunc}$=10, $k_\textrm{top}$=10) & 200 & {100.0} & {0.049} & {0.002} \\
%\bottomrule
%%\midrule
%%\gls{SAB} (no MU) ($k_\textrm{trunc}$=5, $k_\textrm{top}$=5)   & 200 & {\bf 100.0} & {\bf 3.83e-5} & {\bf  4.74e-5} \\
%\end{tabular}
%\end{center}
%%\vspace{-1\baselineskip}
%\vspace{-1mm}
%\caption{Test accuracy and cross-entropy loss performance on the {\bf copying task} with sequence lengths of $T = 200$. Different configurations of \gls{SAB} all reach near optimal performance.}
%\label{tab:copy200}
%\end{table*}
% -----

% ----- original copying T=300 table
%\begin{table*}[h!]
%\footnotesize
%\label{copy300}
%\centering
%\begin{tabular}{l||cccc}
%\toprule
%\textbf{Method} &  \textbf{ Length (T)} & \textbf{Accuracy ($\%$)} &  \textbf{   CE (last 10 chars)} & \textbf{CE}   \\ 
%\midrule
%LSTM (full BPTT) & 300 & 35.9 & 0.197 & 0.047 \\
%LSTM (full selfattention) & 300 & 100.0 & 0.002 & 7.534e-5  \\
%\midrule
%LSTM (TBTT, $k_\textrm{trunc}$= 1) & 300 & 14.0 & 2.077 & 0.065  \\ 
%LSTM (TBPTT, $k_\textrm{trunc}$= 20) & 300 & 25.7  & 1.848 & 0.197 \\
%LSTM (TBPTT, $k_\textrm{trunc}$= 150) & 300 & 24.4 & 1.857 & 0.058\\ 
%\midrule
%\gls{SAB} ($k_\textrm{trunc}$=1, $k_\textrm{top}$=1)   & 300 & 43.1  & 0.231 & 0.045    \\
%%TODO: rerun this experiment, did not converge! need to run for 30 epochs!
%%\gls{SAB} ($k_\textrm{trunc}$=1, $k_\textrm{top}$=1)   & 300 & 26.7  & 0.27 & 0.059    \\
%\gls{SAB} ($k_\textrm{trunc}$=1, $k_\textrm{top}$=5)   & 300 & 89.1  & 0.383  & 0.012  \\
%%\gls{SAB} ($k_\textrm{trunc}$=1, $k_\textrm{top}$=5)   & 300 & 46.5  & 1.340  & 0.042  \\
%\gls{SAB} ($k_\textrm{trunc}$=5, $k_\textrm{top}$=5)   & 300 &  {\bf99.9} & {\bf0.007} & {\bf0.001}   \\
%%\gls{SAB} ($k_\textrm{trunc}$=5, $k_\textrm{top}$=5)   & 300 &  {\bf98.9} & {\bf0.048} & {\bf0.002}   \\
%\bottomrule
%\end{tabular}
%%\vspace{-1\baselineskip}
%\vspace{-1mm}
%\caption{Test accuracy and cross-entropy loss performance on {\bf copying task} with sequence lengths of $T = 300$. On these long sequences  \gls{SAB}'s performance can still be very close to optimal.}
%\label{tab:copy300}
%\vspace{-1\baselineskip}
%\end{table*}
% ----





% ----- original adding table, t=200
%\begin{table}[h!]
%\label{adding200}
%\centering
%\footnotesize
%\begin{tabular}{l||cc}
%\toprule
%\textbf{ Method} &  \textbf{  Length (T)} & \textbf{CE}   \\ 
%\midrule
%LSTM (full BPTT) & 200  &  4.59e-6\\
%LSTM (full selfattention) & 200 & 5.541e-8 \\
%\midrule
%LSTM (TBPTT, $k_\textrm{trunc}$= 20) & 200 &  0.0011\\ 
%LSTM (TBPTT, $k_\textrm{trunc}$=50) & 200 & 0.0003 \\  
%\midrule
%\gls{SAB} ($k_\textrm{trunc}$=5, $k_\textrm{top}$=5)   & 200 &  {\bf 0.0}  \\
%\gls{SAB} ($k_\textrm{trunc}$=10, $k_\textrm{top}$=10)   & 200 & {\bf 2.0e-6}  \\
%%0.000002
%%\gls{SAB} ($k_\textrm{trunc}$=10, $k_\textrm{top}$=10)   & 200 & 0.0001  \\
%\midrule
%\gls{SAB} ($k_\textrm{trunc}$=10, $k_\textrm{top}$=all)   & 200 &   \\
%\gls{SAB} (no MU) ($k_\textrm{trunc}$=10, $k_\textrm{top}$=10)   & 200 & 2.171e-6  \\
%\bottomrule
%\end{tabular}
%\caption{Performance on unseen sequences of the $T=200$ {\bf adding task}. We note that all methods have configurations that allow them to perform near optimally.}
%\label{tab:add200}
%\end{table}


% ------- original adding table, t=400
%\begin{table}
%\footnotesize
%\centering
%\begin{tabular}{l||cc}
%\toprule
%\textbf{Method} &   \textbf{ Length (T)} & \textbf{CE}   \\ 
%\midrule
%LSTM (full BPTT) & 400  & 1.5541e-7 \\ 
%LSTM (full attention) & 400 & 4.972e-7 \\
%LSTM (TBPTT, $k_\textrm{trunc}$=100) & 400 & 6.8e-4 \\ 
%\midrule
%\gls{SAB} ($k_\textrm{trunc}$=5, $k_\textrm{top}$=10)   & 400 & 0.00023 \\
%\gls{SAB} ($k_\textrm{trunc}$=10, $k_\textrm{top}$=10)   & 400 &  {\bf 1.001e-5} \\
%%\gls{SAB} ($k_\textrm{trunc}$=10, $k_\textrm{top}$=10, $k_\textrm{att}$=10)   & 400 & 0.00014 \\
%\midrule
%\gls{SAB} (no MU) ($k_\textrm{trunc}$=10, $k_\textrm{top}$=10)   & 400 & 7.318e-5 \\
%\bottomrule
%\end{tabular}
%%\vspace{-1\baselineskip}
%\caption{Performance on unseen sequences of the $T=400$ {\bf adding task}. BPTT slightly outperforms \gls{SAB} which outperforms TBPTT. $k_{att} = 5$ for all \gls{SAB} models}
%\label{tab:add400}
%\end{table}



% -------- original ptb table
%\begin{table}[!h]
%%\label{tab:ptb}
%\small
%\centering
%%\label{ptb-label}
%\setlength\tabcolsep{2.5pt}
%\begin{tabular}{l||c}
%\toprule
%\textbf{Method}   &\textbf{Test BPC} \\ 
%\midrule
%LSTM (full BPTT)        &  1.36 \\
%LSTM (TBPTT, $k_\textrm{trunc}$=1)    & 1.47  \\ 
%LSTM (TBPTT, $k_\textrm{trunc}$=5)    & 1.44    \\ 
%LSTM (TBPTT, $k_\textrm{trunc}$=20)   & 1.40      \\
%\midrule
%\gls{SAB}  ($k_\textrm{trunc}$=10, $k_\textrm{top}$ =10, $k_\textrm{att}$ = 10)    & 1.402 \\  
%\gls{SAB}  ($k_\textrm{trunc}$=20, $k_\textrm{top}$ =5,  $k_\textrm{att}$ = 20)    & 1.394\\
%\gls{SAB}  ($k_\textrm{trunc}$=20, $k_\textrm{top}$ =10,  $k_\textrm{att}$ = 20)    & 1.37\\
%\bottomrule
%\end{tabular}
%%\vspace{-1\baselineskip}
%\caption{BPC evaluation on the test set of the character-level PTB (lower is better). }
%\label{tab:ptb}
%\end{table}


% ----- original text8 table
%\begin{table}[h!]
%\small
%\centering
%\begin{tabular}{l||c}
%\toprule
%\textbf{Method}  & \textbf{Test BPC}  \\ \midrule
%LSTM (full BPTT)  &  1.48   \\ 
%LSTM (TBPTT, $k_\textrm{trunc}$=5)  &  1.50   \\ 
%\midrule
%\gls{SAB}  ($k_\textrm{trunc}$=10, $k_\textrm{top}$=5, $k_\textrm{att}$=10)   & 1.46    \\ 
%% , attnK = 10
%\bottomrule
%\end{tabular}
%%\vspace{-1\baselineskip}
%\caption{Bit-per-character (BPC) Results on the test set for Text8 (lower is better).}
%\label{tab:text8}
%\vspace{-2mm}
%\end{table}


% ------- original mnist table
%\begin{table}[!htb]
%\small
%\centering
%\setlength\tabcolsep{2.5pt}
%\begin{tabular}{lc}
%\toprule
%\textbf{Method}  & \textbf{Test Acc ($\%$)}  \\
%\midrule
%LSTM (full BPTT)   & 90.3    \\ 
%\hline
%\gls{SAB}  ($k_\textrm{trunc}$=20, $k_\textrm{top}$=5, $k_\textrm{att}$ = 20)   &  89.8    \\ 
%\gls{SAB}  ($k_\textrm{trunc}$=20, $k_\textrm{top}$=10, $k_\textrm{att}$ = 20)   & 90.9    \\
%\gls{SAB}  ($k_\textrm{trunc}$=50, $k_\textrm{top}$=10, $k_\textrm{att}$ = 50)   & {\bf 94.2}    \\ 
%\bottomrule
%\end{tabular}
%\caption{Test and validation accuracy for the permutated MNIST classification task.}
%\label{tab:mnist_seq}
%\end{table}


% -------- original cifar10 table
%\begin{table}[h!]
%\small
%\centering
%\setlength\tabcolsep{2.5pt}
%\begin{tabular}{l||c}
%\toprule
%\textbf{Method}  & \textbf{Test Acc ($\%$)}  \\
%\midrule
%LSTM (full BPTT)   & 58.3   \\ 
%\midrule
%LSTM (truncated BPTT = 300)   & 51.3    \\
%\gls{SAB} & \textbf{64.5}
%\end{tabular}
%
%\caption{Test  accuracy for the CIFAR10 classification task.}
%\label{tab:mnist_seq}
%\end{table}



% ------ original transformer table
%\begin{table}[!h]
%\small
%\centering
%\setlength\tabcolsep{2.5pt}
%\begin{tabular}{l||ccc}
%\toprule
%\textbf{Method} & \textbf{pMNIST} & \textbf{CIFAR10}   \\ 
%\midrule
%Transformer (\cite{DBLP:journals/corr/abs-1803-00144}) & \textbf{97.9} & 62.2     \\ 
%\midrule
%LSTM (\cite{DBLP:journals/corr/abs-1803-00144})  & 89.4 &  58.3\\
%%LSTM (our implementation)  & 90.3 &  60.2\\
%\hline
%Our Model  & 94.2 &  \textbf{64.5}    \\ 
%\bottomrule
%\end{tabular}
%\caption{Test  accuracy for the permutated MNIST and CIFAR10 classification task in comparison to Transformer.}
%\label{tab:transformer}
%\end{table}








% ---------- moved from sect. 4.1
%\textbf{Hyperparameters} The hyperparameters for both baselines and \gls{SAB} are kept the same.  All models has 128 hidden units and uses the Adam \citep{kingma2014adam} optimizer with a learning rate of $1e-3$. The first model in the ablation study (dense version of \gls{SAB}) was more difficult to train, therefore we explored different learning rate ranging from $1e-3$ to $1e-5$, we report the best performing model.

%We study and analyze the performance of \gls{SAB} for 7 different tasks starting from synthetic tasks to test for long-term memory. We first examine the performance of \gls{SAB} on the copying and adding tasks in \cite{hochreiter1997long}, these tasks are designed to measure the model's ability to remember sequences for arbitrary long sequence length. We also provide an ablation study that shows the necessity of sparsity. 

%We now report and discuss the results of an empirical study that analyses the performance of \gls{SAB} using 6 different tasks. We first study synthetic tasks---the copying and adding problems \citep{hochreiter1997long} designed to measure models' abilities to learn long-term dependencies---meant to confirm that \gls{SAB} can successfully perform credit assignment for events that have occurred many time steps in the past. We then study more realistic tasks and larger datasets. 

%\vspace{-2mm}
%\paragraph{Baselines} We compare the quantitative performance of our model against two LSTM baselines \citep{hochreiter1997long}. The first is trained with backpropagation through time (BPTT) and the second is trained using truncated backpropagation through time (TBTPP). Both methods are trained using teacher forcing \citep{williams1989learning}. We also used gradient clipping (that is, we clip the gradients to 1 to avoid exploding gradients). Hyperparameters that are task-specific are discussed in the tasks' respective subsections, other hyperparameters that are also used by \gls{SAB} and that we set to the same value are discussed below. 

%\vspace{-2mm}
%Compared to standard RNNs, our model has two additional hyperparameters:
%\vspace{-3mm}
%\begin{itemize}[noitemsep]
%    \item $k_\textrm{top}$, the number of most-salient microstates to select at each time step for passing gradients in the backward pass
%    \item $k_\textrm{att}$, the granularity of attention. Every $k_\textrm{att}$th hidden state is chosen to be a microstate. The special case $k_\textrm{att} = 1$ corresponds to choosing all hidden states to be microstates as well. 
    %LC: point to the model figure here. 
%\end{itemize}
%\vspace{-3mm}
%In addition, we also study the impact of the TBPTT truncation length, which we denote as $k_\textrm{trunc}$. This determines how many timesteps backwards to propagate gradients through in the backward pass. This effect of this hyperparameter will also be studies for the LSTM with TBTPP baseline. 

%For all experiments we used a learning rate of $0.001$ with the Adam \citep{kingma2014adam} optimizer unless otherwise stated. For \gls{SAB}, we attend to every second hidden states, i.e. $k_\textrm{att}$=2, unless otherwise stated.


%Our main findings are: 
%\begin{enumerate}[noitemsep]
 %   \vspace{-2mm}
%    \item \gls{SAB} performs almost optimally and significantly outperforms both full backpropagtion through time (BPTT), and truncated backpropagation through time (TBPTT) on the synthetic copying task.
%    \item For the synthetic adding, two language modelling task (using PennTree Bank and Text8), and permuted sequential MNIST classification tasks, \gls{SAB} reaches the performance of BPTT and outperforms TBPTT. In addition, for the adding task, \gls{SAB} outperforms TBPTT using much shorter truncation lengths.
%\end{enumerate}
    

% end --------------- moved from sect. 4.1

